Higher finiteness properties of reductive arithmetic groups in positive characteristic: the rank theorem

We show that the finiteness length of an $S$-arithmetic subgroup $\Gamma$ in a noncommutative isotropic absolutely almost simple group $G$ over a global function field is one less than the sum of the local ranks of $G$ taken over the places in $S$. This determines the finiteness properties for arithmetic subgroups in isotropic reductive groups, confirming the conjectured finiteness properties for this class of groups. Our main tool is Behr-Harder reduction theory which we recast in terms of the metric structure of euclidean buildings.

==> basic_notation.tex <==
\ProvidesFile{basic_notation.tex}[2001/09/20 KUB]

%
% This should be merged with buxmath.sty at some point
%

\newcommand{\congruent}[1][]{\equiv_{#1}}


\newcommand{\DisplayOrList}[1]{%
  \ifNotationlisting
    \(#1\)%
  \else
    \[#1\]%
  \fi
}

%
% labelling defining occurences
%
\newcommand{\defnotion}[1]{%
  \begingroup
%    \def\tmp{#1}%
%    \expandafter\label\expandafter{\meaning\tmp}%
    \notion{#1}%
  \endgroup
}
\newcommand{\defref}[1]{%
  \begingroup
    \def\tmp{#1}%
    \expandafter\ref\expandafter{\meaning\tmp}%
  \endgroup
}
\newcommand{\defpref}[1]{%
  (\defref{#1})%
}
\newcommand{\locnotion}[1]{\emph{#1}}

%
% vertical =
%
\newcommand{\veq}{\shortparallel}

%
% set theory
%

\newcommand{\union}{\cup\OptIndex}
\newcommand{\symmetricdifference}{\mathbin{\triangle}}%{\mathbin{+_\Two}}
\newcommand{\intersect}[1][]{\cap_{#1}}
%\newcommand{\disjointunion}{\,\,\hbox to 0pt{$\hss\cdot\hss$}\hbox to 0pt{$\hss\union\hss$}\,\,}
\newcommand{\disjointunion}{\uplus}
\newcommand{\equalls}[1][]{%
  \IfEmptyThenElse{#1}{%
    =
  }{%
    =_{#1}
  }
}

\newcommand{\getparfirstarg}[1][]{%
  \def\tempa{#1}%
  \getparsecondarg
}
\newcommand{\getparsecondarg}[1][]{%
  \def\tempb{#1}%
  \processparcmd
}
\newcommand{\processparcmd}[1]{%
  \parcmd{#1}{\tempa}{\tempb}\endgroup
}
\newcommand{\doparcmd}[1]{%
  \begingroup
    \def\parcmd{#1}%
    \getparfirstarg
}
\newcommand{\parentheses}[3]{%
  {\left({#1}\right)_{#2}^{#3}}%
}
\newcommand{\Parentheses}{%
  \doparcmd{\parentheses}%
}
\newcommand{\OldParentheses}[1]{\left(#1\right)}
\newcommand{\ParenthesesDouble}[1]{\left(\left(#1\right)\right)}
\newcommand{\Brakets}[1]{\left[#1\right]}
\newcommand{\BraketsDouble}[1]{\left[\left[#1\right]\right]}
\newcommand{\ToThePower}[2]{{#1}^{#2}}
\newcommand{\AbsValue}[1]{\left|#1\right|}
\newcommand{\Factorial}[1]{#1!}

\newcommand{\EvalAt}{\negthinspace\OldParentheses}
\newcommand{\EvalAtAt}{\negthinspace\ParenthesesDouble}
\newcommand{\EvalAd}{\negthinspace\Brakets}
\newcommand{\EvalAdAd}{\negthinspace\BraketsDouble}
\newcommand{\ImageAt}{\negthinspace\OldParentheses}
\newcommand{\ActOn}{\cdot}
\newcommand{\RestrictionTo}[1]{|_{#1}}

\newcommand{\OpenInterval}[2]{\left(#1,#2\right)}
\newcommand{\ClosedInterval}[2]{\left[#1,#2\right]}
\newcommand{\RightOpenInterval}[2]{\left[#1,#2\right)}
\newcommand{\LeftOpenInterval}[2]{\left(#1,#2\right]}

\newcommand{\Binom}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)}

\newcommand{\gobbleopt}[1][]{}

\newcommand{\forinf}{\exists^\infty}
\newcommand{\Forsome}[1]{\text{\ for some\ }#1}
\newcommand{\Forall}[1]{\text{\ for all\ }#1}
\newcommand{\Forinfmany}[1]{\qquad\text{\ for infinitely many\ }#1}
\newcommand{\ForSome}[1]{\qquad\text{\ for some\ }#1}
\newcommand{\ForAll}[1]{\qquad\text{\ for all\ }#1}
\newcommand{\ForInfMany}[1]{\qquad\text{\ for infinitely many\ }#1}
\newcommand{\For}[1]{\qquad\text{\ for\ }#1}
\newcommand{\Since}[1]{\qquad\text{\ since\ }#1}
\newcommand{\With}[1]{\qquad\text{\ with\ }#1}
\newcommand{\As}[1]{\qquad\text{\ as\ }#1}
%\newcommand{\AND}{\qquad\text{\ and\ }\qquad}
%\newcommand{\OR}{\qquad\text{\ or\ }\qquad}
%\newcommand{\IF}{\qquad\text{\ if\ }\qquad}
\newcommand{\IFF}{\qquad\text{\ if and only if\ }\qquad}
\newcommand{\DefIff}{:\Longleftrightarrow}
\newcommand{\Iff}{\ensuremath{\Longleftrightarrow}}
\newcommand{\Implies}{\ensuremath{\Longrightarrow}}

\newcommand{\ExtPowerOf}[2][]{%
  \ExtPot^{#1}\left(#2\right)
}
\newcommand{\tensor}[1][]{\otimes_{#1}}
\newcommand{\BilOf}[2][]{%
  \operatorname{Bil}_{#1}\negthinspace\left(#2\right)
}
\newcommand{\ExpOf}[2][]{\mathop{\exp_{#1}}\negthinspace\left(#2\right)}

\newcommand{\Diff}[1]{\mathrm{d}#1}
\newcommand{\Brace}[3]{%
  \left[#3\right]_{#1}^{#2}
}

\newcommand{\mapcolon}{:}

%
% Compound Notations
%
\makeatletter
\newcommand{\TwoByTwoMatrix}[4]{%
%    \left(\begin{array}{cc}
  \begin{pmatrix}
      #1 & #2\\
      #3 & #4
  \end{pmatrix}
%    \end{array}\right)
}

\newcommand{\TwoByTwoDet}[4]{%
    \left|\begin{array}{cc}
      #1 & #2\\
      #3 & #4
    \end{array}\right|
}

\newcommand{\TwoColVector}[2]{%
    \left(\begin{array}{cc}
      #1\\
      #2
    \end{array}\right)
}

\newcommand{\TwoRwoVector}[2]{%
  \OldParentheses{#1,#2}
}
\providecommand{\IfEmptyThenElse}[1]{%
  \begingroup
    \def\tempa{#1}%
    \def\tempb{}%
    \ifx\tempa\tempb
      \def\next{\@firstoftwo}%
    \else
      \def\next{\@secondoftwo}%
    \fi
  \expandafter\endgroup\next
}

\newcommand{\getsetfamfirstarg}[1][]{
  \def\tempa{#1}%
  \getsetfamsecondarg
}
\newcommand{\getsetfamsecondarg}[2][]{
  \def\tempb{#1}%
  \def\empty{}%
  \ifx\tempa\empty
    \left(#2\right)%
  \else
    \ifx\tempb\empty
      \left\{#2\right\}_{\tempa}%
    \else
      \left\{#2\right\}_{\tempa}^{\tempb}%
    \fi
  \fi
  \endgroup
}
\newcommand{\SetFamOf}{%
  \begingroup
    \getsetfamfirstarg
}

\newcommand{\getfamfirstarg}[1][]{
  \def\tempa{#1}%
  \getfamsecondarg
}
\newcommand{\getfamsecondarg}[2][]{
  \def\tempb{#1}%
  \def\empty{}%
  \ifx\tempa\empty
    \left(#2\right)%
  \else
    \ifx\tempb\empty
      \left(#2\right)_{\tempa}%
    \else
      \left(#2\right)_{\tempa}^{\tempb}%
    \fi
  \fi
  \endgroup
}
\newcommand{\FamOf}{%
  \begingroup
    \getfamfirstarg
}
\iffalse
\newcommand{\FamOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \left(#2\right)
  }{
    \left(#2\right)_{#1}
  }
}
\fi

\newcommand{\SetOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \left\{#2\right\}
  }{
    \left\{#1\,\,\vrule\,\,#2\right\}
  }
}

\newcommand{\GroupPresented}[2][]{%
  \IfEmptyThenElse{#1}{
    \left\langle#2\right\rangle
  }{
    \left\langle#1\,\,\vrule\,\,#2\right\rangle
  }
}
\newcommand{\EquivClassOf}[2][]{\left[#2\right]_{#1}}
\newcommand{\TupelOf}[2][]{\left(#2\right)_{#1}}
\newcommand{\MaxOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \max\left(#2\right)
  }{
    \max_{#1}\left(#2\right)
  }
}

\newcommand{\SupOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \operatorname{sup}\left(#2\right)
  }{
    \operatorname{sup}_{#1}\left(#2\right)
  }
}

\newcommand{\MinOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \min\left(#2\right)
  }{
    \min_{#1}\left(#2\right)
  }
}

\newcommand{\InitTripleCommand}[2][]{%
  \begingroup
    \def\EndSymbol{#1}
    \def\TheSymbol{#2}%
    \getfirstarg
}
\newcommand{\getfirstarg}[1][]{%
    \def\tempa{#1}%
    \getlastargs
  }
\newcommand{\getlastargs}[2][]{%
    \def\tempb{#1}%
    \def\empty{}%
    \ifx\tempb\empty
      \ifx\tempa\empty
        \TheSymbol #2%
      \else
        \TheSymbol_{\tempa}#2%
      \fi
    \else
      \TheSymbol_{\tempa}^{#1}#2%
    \fi
  \endgroup
}

\newcommand{\Lim}[2][]{\lim_{#1}#2}

\newcommand{\Sum}[0]{\InitTripleCommand{\sum}}
\newcommand{\Int}[0]{\InitTripleCommand{\int}}
\newcommand{\Union}[0]{\InitTripleCommand{\bigcup}}
\newcommand{\Intersection}[0]{\InitTripleCommand{\bigcap}}
\newcommand{\DisUnion}[0]{\InitTripleCommand{{\biguplus}}}
\newcommand{\Product}[0]{\InitTripleCommand{\prod}}
\newcommand{\CoProduct}[0]{\InitTripleCommand{\coprod}}
\newcommand{\XProduct}[0]{\InitTripleCommand{\bigtimes}}
\newcommand{\FreeProd}[0]{\InitTripleCommand{\bigast}}
\newcommand{\BigJoin}[0]{\InitTripleCommand{\bigast}}
\newcommand{\DirectSum}[0]{\InitTripleCommand{\bigoplus}}
\newcommand{\Min}[0]{\InitTripleCommand{\min}}
\newcommand{\Max}[0]{\InitTripleCommand{\max}}
\newcommand{\Inf}[0]{\InitTripleCommand{\inf}}
\newcommand{\InfOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \inf#2
  }{
    \inf_{#1}#2
  }
}
\newcommand{\Sup}[0]{\InitTripleCommand{\sup}}

\newcommand{\MatrixOf}[2][]{%
  \IfEmptyThenElse{#1}{%
    \left(#2\right)
  }{%
    \left(#2\right)_{#1}
  }
}

\newcommand{\OrderOf}{\operatorname{ord}\OptIndexParentheses}

\newcommand{\TensorProduct}[3][]{%
  \IfEmptyThenElse{#1}{
    #2\otimes#3
  }{
    #2\otimes_{#1}#3
  }
}

\newcommand{\leftsemidirectprod}[1][]{%
  \rtimes\OptIndex[#1]
}

\newcommand{\wreathprod}{\wr}

\newcommand{\ColumnVector}[1]{%
  \left(\begin{array}{c}
    #1
  \end{array}\right)
}

\newcommand{\Interval}[2]{\left[#1,#2\right]}

% \makeatletter
% \def\@lap[#1,#2]#3{%
%   \parbox[b][0pt][b]{0pt}{%
%     \raisebox{#2}{%
%       \parbox[b][0pt][c]{0pt}{%
%          \makebox[0pt][c]{\null\kern#1\kern#1{#3}}%
%       }%
%     }%
%   }%
%   \ignorespaces
% }%
% \newcommand{\clap}[2][0pt,0pt]{\@lap[#1]{#2}}
% \makeatother

\newcommand{\clap}[1]{\makebox[0pt][c]{#1}}


\newcommand{\PreImage}[2]{{#1}^{-1}\left(#2\right)}
%
%
%
\newcommand{\IfNonEmpty}[2]{\IfEmptyThenElse{#1}{}{#2}}
\newcommand{\OptExponent}[1][]{\IfNonEmpty{#1}{^{#1}}}
\newcommand{\OptParExponent}[1][]{\IfNonEmpty{#1}{^{\left(#1\right)}}}
\newcommand{\OptIndex}[1][]{\IfNonEmpty{#1}{_{#1}}}
\newcommand{\OptArg}[2]{#1\IfNonEmpty{#2}{\EvalAt{#2}}}
\newcommand{\OptIndexOptPar}[1][]{\IfNonEmpty{#1}{_{#1}}\OptParentheses}
\newcommand{\OptParentheses}[1][]{\IfNonEmpty{#1}{\negthinspace\left(#1\right)}}
\newcommand{\OptExponentParentheses}[1][]{\IfNonEmpty{#1}{^{#1}}\EvalAt}
\newcommand{\OptExponentParenthesesDouble}[1][]{\IfNonEmpty{#1}{^{#1}}\EvalAtAt}
\newcommand{\OptExponentBrakets}[1][]{\IfNonEmpty{#1}{^{#1}}\EvalAd}
\newcommand{\OptExponentBraketsDouble}[1][]{\IfNonEmpty{#1}{^{#1}}\EvalAdAd}
\newcommand{\OptIndexParentheses}[1][]{\IfNonEmpty{#1}{_{#1}}\OptExponentParentheses}
\newcommand{\OptIndexParenthesesDouble}[1][]{\IfNonEmpty{#1}{_{#1}}\OptExponentParenthesesDouble}
\newcommand{\OptIndexBrakets}[1][]{\IfNonEmpty{#1}{_{#1}}\OptExponentBrakets}
\newcommand{\OptIndexBraketsDouble}[1][]{\IfNonEmpty{#1}{_{#1}}\OptExponentBraketsDouble}
\newcommand{\OptIndexParExponent}[1][]{\IfNonEmpty{#1}{_{#1}}\OptParExponent}
\newcommand{\OptIndexExponent}[1][]{\IfNonEmpty{#1}{_{#1}}\OptExponent}
\newcommand{\DoubleArg}[2]{\EvalAt{#1,#2}}
\newcommand{\OptExponentDoubleArg}[1][]{\IfNonEmpty{#1}{_{#1}}\DoubleArg}
\newcommand{\OptIndexDoubleArg}[1][]{\IfNonEmpty{#1}{_{#1}}\OptExponentDoubleArg}
\newcommand{\newconst}[2]{%
  \newcommand{#1}[0]{#2}
  }
\newcommand{\UnVar}[1]{%
  \let#1\undefined
  \expandafter\let\csname\expandafter\@gobble\string#1Of\endcsname\undefined
  \expandafter\let\csname\expandafter\@gobble\string#1OfOf\endcsname\undefined
  \expandafter\let\csname\expandafter\@gobble\string#1Ad\endcsname\undefined
  \expandafter\let\csname\expandafter\@gobble\string#1AdAd\endcsname\undefined
}
\newcommand{\newvariable}[2]{%
  \newcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\OptExponent}
  \expandafter\newcommand\csname\expandafter\@gobble\string#1Of\endcsname{#1\OptIndexParentheses}
  \expandafter\newcommand\csname\expandafter\@gobble\string#1OfOf\endcsname{#1\OptIndexParenthesesDouble}
  \expandafter\newcommand\csname\expandafter\@gobble\string#1Ad\endcsname{#1\OptIndexBrakets}
  \expandafter\newcommand\csname\expandafter\@gobble\string#1AdAd\endcsname{#1\OptIndexBraketsDouble}
  }
\newcommand{\renewvariable}[2]{%
  \renewcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\OptExponent}
  \expandafter\renewcommand\csname\expandafter\@gobble\string#1Of\endcsname{#1\OptIndexParentheses}
  \expandafter\renewcommand\csname\expandafter\@gobble\string#1Ad\endcsname{#1\OptIndexBrakets}
}
%\newcommand{\renewvariable}[1]{%
%  \glet#1\undefined
%  \expandafter\glet\csname\expandafter\@gobble\string#1Of\endcsname\undefined
%  \expandafter\glet\csname\expandafter\@gobble\string#1Ad\endcsname\undefined
%  \newvariable#1
%}
\newcommand{\tmpvariable}[2]{%
  \let#1\undefined
  \expandafter\let\csname\expandafter\@gobble\string#1Of\endcsname\undefined
  \newcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\OptExponent}
  \expandafter\newcommand\csname\expandafter\@gobble\string#1Of\endcsname{#1\OptIndexParentheses}
  }
\newcommand{\newparexpvariable}[2]{%
  \newcommand{#1}{#2\OptIndexParExponent}
  }
\newcommand{\newmap}[2]{%
  \newcommand{#1}[1][]{\OptArg{#2}{##1}}
  }
\newcommand{\newindexedmap}[2]{%
  \newcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\OptParentheses}
  }
\newcommand{\NewMap}[2]{%
  \newvariable{#1}{#2}%
  \begingroup
    \escapechar=-1%
    \expandafter\global\expandafter\newcommand\expandafter{\csname \string#1Of\endcsname}{#2\OptIndexParentheses}
  \endgroup
}
\newcommand{\newMap}[2]{%
  \newcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\EvalAt}
  }
\newcommand{\newMapTwo}[2]{%
  \newcommand{#1}[2]{#2\left(##1,##2\right)}
  }
\newcommand{\newMapTWO}[2]{%
  \newcommand{#1}[2]{#2\left(##1;##2\right)}
  }
\newcommand{\newexpvector}[2]{%
  \newcommand{#1}{#2\OptParExponent}
  }

\newcommand{\newexpvar}[2]{%
  \newcommand{#1}{#2\OptIndexExponent}
}
\newcommand{\newparexpvar}[2]{%
  \newcommand{#1}{#2\OptIndexParExponent}
}
\newcommand{\OR}{\quad\text{or}\quad}
%
% picture
%
  \newcommand{\drawpath}[1]{%
    \begingroup%
      \edef\tempa{#1}%
      \expandafter\drawline\tempa%
    \endgroup%
    \ignorespaces
  }
  \newcommand{\dashpath}[2]{%
    \begingroup%
      \edef\tempa{#2}%
      \def\tempb{\dashline[0]{#1}}%
      \expandafter\tempb\tempa%
    \endgroup%
    \ignorespaces
  }
  \newcommand{\plot}[2]{%
    \expandafter\put#1{#2}\ignorespaces
  }
  \def\lap[#1,#2]#3{%
    \parbox[b][0pt][b]{0pt}{%
      \raisebox{#2}{%
        \parbox[b][0pt][c]{0pt}{%
           \makebox[0pt][c]{\null\kern#1\kern#1{#3}}%
        }%
      }%
    }%
    \ignorespaces
  }%
  \newcommand{\Bullet}[2][0mm,0mm]{%
    \lap[0mm,0mm]{$\bullet$}
    \lap[#1]{$#2$}
  }

\newcommand{\UnitsOf}[1]{#1^{*}}
\newcommand{\ThePullback}[1]{#1^{*}\OptParentheses}

\newcommand{\DirectedSystem}[3][]{%
  \IfEmptyThenElse{#1}{%
    (#2)_{#3}
  }{%
    (#2)_{#1\in#3}%
  }%
}

\newcommand{\Morph}[3][]{%
  \IfEmptyThenElse{#1}{%
    \mathop{\mathrm{Mor}}\left(#2,#3\right)%
  }{%
    \mathop{\mathrm{Mor}}\limits_{#1}\left(#2,#3\right)%
  }%
}
\newcommand{\InvLimit}[2][]{\mathop{\inverslim}_{#1}#2}
\newindexedmap{\InvLimitMap}{\pi}
\newmap{\InvUnivMap}{\iota}
\newcommand{\DirLimit}[2][]{\mathop{\directlim}_{#1}#2}
\newindexedmap{\DirLimitMap}{\iota}
\newmap{\DirUnivMap}{\pi}
\newcommand{\Limit}[2][]{\mathop{\lim}_{#1}#2}

\newcommand{\HoColimOf}[1]{%
  \operatorname{ho-colim}\left(#1\right)
}

\newcommand{\FunctorMap}[1]{#1_{*}\OptParentheses}
\newvariable{\TheGraphLift}{\tilde{\TheGraph}}
\newcommand{\graphminus}{-}
\newvariable{\TheEdgeLift}{\tilde{\TheEdge}}

%
% small integers
%
\newcommand{\Number}[1]{#1}
\newvariable{\Zero}{\Number{0}}
\newvariable{\One}{\Number{1}}
\newvariable{\qOne}{1}
\newvariable{\OneHalf}{\ensuremath{\frac{1}{2}}}
\newvariable{\Two}{\Number{2}}
\newvariable{\Three}{\Number{3}}
\newvariable{\Four}{\Number{4}}
\newvariable{\Five}{\Number{5}}
\newvariable{\Six}{\Number{6}}
\newvariable{\Seven}{\Number{7}}
\newvariable{\Eight}{\Number{8}}
\newvariable{\Nine}{\Number{9}}
\newvariable{\Ten}{\Number{10}}
\newvariable{\Eleven}{\Number{11}}
\newvariable{\Twelve}{\Number{12}}

%
% Group Actions
%
\newcommand{\ActingOn}{\negthinspace.}
\newcommand{\ActsOn}{\curvearrowright}

\endinput

